At the Dawn of Generative AI Era: A Tutorial-cum-Survey on New Frontiers in 6G Wireless Intelligence

The majority of data-driven wireless research leans heavily on discriminative AI (DAI) that requires vast real-world datasets. Unlike the DAI, Generative AI (GenAI) pertains to generative models (GMs) capable of discerning the underlying data distribution, patterns, and features of the input data. This makes GenAI a crucial asset in wireless domain wherein real-world data is often scarce, incomplete, costly to acquire, and hard to model or comprehend. With these appealing attributes, GenAI can replace or supplement DAI methods in various capacities. Accordingly, this combined tutorial-survey paper commences with preliminaries of 6G and wireless intelligence by outlining candidate 6G applications and services, presenting a taxonomy of state-of-the-art DAI models, exemplifying prominent DAI use cases, and elucidating the multifaceted ways through which GenAI enhances DAI. Subsequently, we present a tutorial on GMs by spotlighting seminal examples such as generative adversarial networks, variational autoencoders, flow-based GMs, diffusion-based GMs, generative transformers, large language models, to name a few. Contrary to the prevailing belief that GenAI is a nascent trend, our exhaustive review of approximately 120 technical papers demonstrates the scope of research across core wireless research areas, including physical layer design; network optimization, organization, and management; network traffic analytics; cross-layer network security; and localization & positioning. Furthermore, we outline the central role of GMs in pioneering areas of 6G network research, including semantic/THz/near-field communications, ISAC, extremely large antenna arrays, digital twins, AI-generated content services, mobile edge computing and edge AI, adversarial ML, and trustworthy AI. Lastly, we shed light on the multifarious challenges ahead, suggesting potential strategies and promising remedies.

==> tables/Table_GAN_NIDS.tex <==
\begin{table*}[htbp]
\caption{Summary of GAN-based Network Intrusion Detection Systems}
\label{tab:summary_gan_ids}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Paper}                           & \textbf{Key Focus}              & \textbf{Approach / Model}          & \textbf{Dataset(s)}                     & \textbf{Key Findings}                                                                                \\ \hline
\cite{vu2023nids}       & Cloud environment               & CDAEE-KNN models                   & Four popular NIDS datasets               & Improved accuracy and robustness in detecting diverse attacks   \\ \hline
\cite{gao2014nids}      & Big Data classification         & DBNs                               & KDD CUP 1999 dataset                    & Outperformed SVM and ANN in intrusion detection                                                      \\ \hline
\cite{seo2018nids}      & In-vehicle networks             & GAN-based NIDS                     & In-vehicle network dataset              & High detection accuracy for four unknown attacks                                                     \\ \hline
\cite{ding2022nids}     & Imbalanced learning             & TACGAN                             & Three real NIDS datasets & Achieved excellent results in Accuracy, F1, AUC, and Recall                                          \\ \hline
\cite{park2023nids}     & Data imbalance                  & GANs and AE-driven models          & Various datasets                        & Significant improvement in AI-based NIDS performance                                                 \\ \hline
\cite{huang2020nids}    & Class imbalance                 & Imbalanced GAN                     & Three benchmark datasets                & Outperformed 15 other methods, demonstrating effectiveness of IGAN-IDS                               \\ \hline
\cite{jeong2021nids}    & Semi-supervised learning        & SS-GAN                             & CICIDS-2017 dataset                     & Outperformed other malware traffic classification models                                             \\ \hline
\cite{salem2018nids}    & Anomaly generation              & Cycle-GAN                          & ADFA-LD dataset                         & Improved AUC from 0.55 to 0.71, anomaly detection rate from 17.07\% to 80.49\%                       \\ \hline
\cite{usama2019nids}    & Adversarial ML attack           & GANs for evasion and inoculation   & Not specified                           & Improved robustness to adversarial perturbations \\ \hline
\cite{creech2014nids}   & Host-based anomaly detection    & Discontiguous system call patterns & KDD98, UNM, and ADFA Linux              & Improved/reduced detection/false-alarm, inherent resilience to mimicry attacks      \\ \hline
\cite{freitas2021nids}  & Low-latency IDS for CPSs        & FID-GAN in a fog architecture      & Three studied datasets                  & Achieved higher detection rates faster           \\ \hline
\cite{ferdowsi2019nids} & Distributed GAN for IoT         & Distributed GAN-based NIDS         & Not specified                           & Up to 20\% higher accuracy, 25\% higher precision, and 60\% lower false positive rate                \\ \hline
\cite{shahriar2020nids} & Imbalanced/missing CPS data & GAN-based NIDS                         & NSL KDD-99 dataset                      & Improved attack detection and model stabilization \\ \hline
\end{tabular}
}
\end{table*}


==> tables/Table_GM_Comp_highlevel.tex <==

\begin{table}[t!]
\centering
\caption{High-level comparison of GMs}
\label{tab:GM_highlevel}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\textbf{Criterion} & \textbf{GANs} & \textbf{VAEs} & \textbf{GAMs} & \textbf{RBMs} & \textbf{DBNs} & \textbf{FGMs} & \textbf{DGMs} \\ \hline
Sample Quality        & High   & Medium & High   & Medium & Medium & High   & High   \\ \hline
Training Stability    & Low    & High   & Medium & High   & High   & High   & Medium \\ \hline
Inference Speed       & High   & High   & Medium & High   & High   & High   & Medium \\ \hline
Scalability           & High   & High   & High   & Medium & Medium & High   & High   \\ \hline
Expressiveness        & High   & High   & High   & Medium & Medium & High   & High   \\ \hline
Disentanglement      & Medium & High   & Medium & Low    & Low    & Medium & Medium \\ \hline
Ease of Training      & Medium & High   & Medium & High   & Medium & High   & Medium \\ \hline
Evaluation Metrics    & Medium & High   & High   & High   & High   & High   & High   \\ \hline
Interpretability      & Low    & Medium & Medium & Medium & Medium & Medium & Medium \\ \hline
Cond. Generation& High   & High   & High   & Medium & Medium & High   & High   \\ \hline
\end{tabular}
}

\end{table}


==> tables/Table_Localization.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\centering
\caption{Generative Models Used for Localization and Positioning}
\label{tab:localization}
\resizebox{1.35\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Ref.} &
  \textbf{Year} &
  \textbf{Key Concept} &
  \textbf{Model Used} &
  \textbf{Data Collection} &
  \textbf{Benefits/Improvements} &
  \textbf{Benchmarks} \\ \hline
\cite{ren2021loc} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}Overcoming time-consuming manually updates of the WiFi fingerprint database by\\ rebuilding missing fingerprints by predicting residual RSS based on random sampling\end{tabular} &
  Tensor-GAN &
  Real-world fingerprint data set &
  Localization accuracy improved by 80\% of 1639 random testing points. &
  kNN, DeepFi, AutoEncoder \\ \hline
\cite{zhou2020loc} &
  2020 &
  \begin{tabular}[c]{@{}l@{}}Mitigating traditional time-consuming radio map construction to automate radio map \\ creation for WLAN-based target intrusion sensing and localization\end{tabular} &
  ACO-GAN &
  WiFi  RSSI fingerprint database &
  \begin{tabular}[c]{@{}l@{}}Efficient and accurate rebuilding of missing fingerprints, robustness to \\ time consumption on the learning progress\end{tabular} &
  Not specified \\ \hline
\cite{njima2021loc} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}SSL based data augmentation to alleviate data insufficiency in indoor localization by \\ utilizing GANs to generate fake fingerprints from a small dataset\end{tabular} &
  RaGAM &
  Actual unlabeled RSSI data &
  \begin{tabular}[c]{@{}l@{}}Reduction in labor and time cost, improved computation cost \\ and ray-tracing accuracy, accurate target intrusion sensing\end{tabular} &
  Not specified \\ \hline
\cite{njima2021loc_journal} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}Proposing a generation/selection of fake RSSI data to cover the entire indoor environment \\ and reduce the data generation error by only selecting the most realistic fake RSSIs\end{tabular} &
  GAN, DNN &
  Labeled and unlabeled fingerprints &
  \begin{tabular}[c]{@{}l@{}}Mean localization accuracy improvement of 9.66\% compared \\ to the conventional semi-supervised localization algorithm\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Semi-supervised \\ Localization\end{tabular} \\ \hline
\cite{njima2022loc} &
  2022 &
  \begin{tabular}[c]{@{}l@{}}Addressing the limited labeled data and its impact on localization accuracy by \\ generating fake fingerprints using weighted GANs\end{tabular} &
  Weighted GAN &
  Small set of real labeled data &
  \begin{tabular}[c]{@{}l@{}}Localization accuracy improvement of 21.69\% for simulated data \\ and 15.36\% for experimental data\end{tabular} &
  Not specified \\ \hline
\cite{suroso2022loc} &
  2022 &
  \begin{tabular}[c]{@{}l@{}}Alleviating the drawbacks of long effort and high cost of constructing offline database \\ issues and overcome RSSI fluctuation and instability.\end{tabular} &
  VAEs &
  Real and synthetic data &
  \begin{tabular}[c]{@{}l@{}}Improved accuracy by 10.11\%-8.53\% compared to the classical DL \\ method using the same set of labeled collected data.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Classical SL \\ Method\end{tabular} \\ \hline
\cite{alberto2020loc} &
  2020 &
  \begin{tabular}[c]{@{}l@{}}Using recurrent models to learn the human movement based on sensors and using GAN \\ for data generation and recovery Adaptive indoor person tracking using wireless sensors\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}RecTrack-GAN\\ cGAN\end{tabular} &
  RSSI Fingerprinting database &
  \begin{tabular}[c]{@{}l@{}}Improvement in accuracy performance and reduction in error deviation for \\ tracking up to 15\% compared to the prior art in the literature\end{tabular} &
  Prior art \\ \hline
\cite{li2018locfinger} &
  2018 &
  \begin{tabular}[c]{@{}l@{}}Convert CSI to feature maps using complex wavelet transform, then extend the \\ fingerprint database by the proposed Wavelet Transform-Feature DC-GAN\end{tabular} &
  DC-GAN &
  CSI data at reference points &
  \begin{tabular}[c]{@{}l@{}}Improvement of accuracy of indoor localization system, accelerated \\ convergence in training phase, increased diversity of generated feature maps\end{tabular} &
  N/A \\ \hline
\cite{li2021locfinger} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}Converting CSI data collected at reference point sinto amplitude feature maps and \\ extend the fingerprint database using the proposed Amplitude-Feature DCGAN\end{tabular} &
  AF-DCGAN &
  CSI data at reference points &
  \begin{tabular}[c]{@{}l@{}}Improved accuracy, accelerated training convergence, increased CSI amplitude \\ feature map diversity, reduced human effort in fingerprint database construction.\end{tabular} &
  N/A \\ \hline
\cite{lim2021locfinger} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}Synthesizing a dense fingerprint map by using GAN to learn a sparse CSI image \\ and interpolate missing values of the sparse CSI data.\end{tabular} &
  GAN &
  CSI at sparse reference points &
  \begin{tabular}[c]{@{}l@{}}Improved localization accuracy with less reference points, \\ GAN creates artificial CSI amplitude data similar to actual samples\end{tabular} &
  N/A \\ \hline
\cite{wei2021locfinger} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}Alleviating the time-intensive data-labeling by constructing CSI amplitude colormaps\\ and generating artificial fingerprint using a single AC-GAN\end{tabular} &
  AC-GAN &
  Raw CSI data at each reference points &
  \begin{tabular}[c]{@{}l@{}}Improved localization accuracy, reduced computing resource consumption, \\ and lower training time with single AC-GAN\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Multi-GAN \\ Approaches\end{tabular} \\ \hline
\cite{zhu2018locfinger} &
  2018 &
  \begin{tabular}[c]{@{}l@{}}A tensor-GANsuper-resolution scheme using that adopts sparse coding as the generator\\ and a residual learning network as the discriminator to model fingerprint samples.\end{tabular} &
  Tensor-GAN &
  Fingerprint samples &
  \begin{tabular}[c]{@{}l@{}}Improved solution in localization accuracy, response time, \\ and implementation complexity compared to existing methods\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Existing smartphones \\ indoor positioning\end{tabular} \\ \hline
\cite{chen2020locfinger} &
  2020 &
  \begin{tabular}[c]{@{}l@{}}Device-free wireless indoor localization using semi-supervised learning approach \\ to considerably reduce the expensive data labeling effort\end{tabular} &
  GAN &
  Small/large labeled/unlabeled data &
  \begin{tabular}[c]{@{}l@{}}Comparable performance with equal, sufficient amount of labeled data, and\\ superior performance with equal, highly limited amount of labeled data\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}State-of-the-art \\ SL Schemes\end{tabular} \\ \hline
\cite{darwin2022locfinger} &
  2022 &
  Indoor Positioning based on Machine Learning &
  \begin{tabular}[c]{@{}l@{}}CNN, LSTM, \\ and GAN\end{tabular} &
  Reference data &
  Positioning error reduced in more than 70\% of 17 public datasets &
  Not specified \\ \hline
\cite{serreli2021locfinger} &
  2021 &
  \begin{tabular}[c]{@{}l@{}}LTE Advanced Fingerprint-based localization approach to mitigate costly \\ and time-consuming offline training phase\end{tabular} &
  GAN &
  RSSI &
  \begin{tabular}[c]{@{}l@{}}Improved accuracy, fast and time-saving measurement campaign, accuracy \\ of 0.4/10 m in indoor/outdoor environments, respectively\end{tabular} &
  Not specified \\ \hline
\cite{tarekegn2020locfinger} &
  2020 &
  \begin{tabular}[c]{@{}l@{}}Fingerprint-based IoT positioning to minimize the site survey time/cost \\ to create a radio map and to mitigate signal fluctuations\end{tabular} &
  DCGANs &
  WLAN/Cellular Radio Signals &
  \begin{tabular}[c]{@{}l@{}}Promising and reasonable positioning performance for \\ IoT devices in scalable wireless environments\end{tabular} &
  Not specified \\ \hline
\cite{hua2021locvlc} &
  2021 &
  Li-Fi indoor positioning system &
  \begin{tabular}[c]{@{}l@{}}Adversarial\\ Networks\end{tabular} &
  Not specified &
  \begin{tabular}[c]{@{}l@{}}Significant improvement in challenging environment compared to\\ traditional least square algorithm\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Least Square\\ Estimation\end{tabular} \\ \hline
\cite{liu2022locvlc} &
  2022 &
  Accurate Li-Fi location estimation for pedestrians &
  GAN &
  GPS, IMU, FTM Data &
  \begin{tabular}[c]{@{}l@{}}1-2 meter localization error across 5 different outdoor scenes, localization \\ accuracy improved by up to 26\% after fine-tuning on the expanded dataset\end{tabular} &
  Not specified \\ \hline
\end{tabular}%
}
\end{table}
\end{landscape}

==> tables/Table_ML_apps.tex <==
% \begin{table}[t!]
%   \centering
%   \caption{ML applications in wireless networks}
%   \label{tab:ML_apps}
%   \resizebox{0.5\textwidth}{!}{%
%   \begin{tabular}{|l|c|c|c|}
%    \hline
%     \textbf{Applications} & \textbf{Supervised} & \textbf{Unsupervised} & \textbf{Reinforcement} \\ \hline
%     Traffic Prediction & \cite{zhou2019deep} & \cite{jiang2018traffic} & $\xmark$ \\ \hline
%     Congestion Control & \cite{cui2019convex} & \cite{chen2018joint} & \cite{wang2019deep} \\ \hline
%     Anomaly Detection & \cite{luo2018distributed} & \cite{cui2019convex} & $\xmark$ \\ \hline
%     CSI Estimation & \cite{he2018deep} & $\xmark$ & $\xmark$ \\ \hline
%     Network Optimization & \cite{sun2019learning} & \cite{wang2019deep} & \cite{wang2019deep} \\ \hline
%     Routing & $\xmark$ & \cite{chen2018joint} & \cite{wang2019deep} \\ \hline
%     Spectrum Management & $\xmark$ & $\xmark$ & \cite{wang2019deep} \\ \hline
%     Handover Management & \cite{nassar2019deep} & $\xmark$ & \cite{nassar2019deep} \\ \hline
%     Resource Allocation & \cite{sun2019learning} & \cite{wang2019deep} & \cite{wang2019deep} \\ \hline
%     Physical Layer Security & \cite{he2018deep} & \cite{cui2019convex} & $\xmark$ \\ \hline
%   \end{tabular}
% }
% \end{table}

\begin{table}[t!]
  \centering
  \caption{ML applications in wireless networks.}
  \label{tab:ML_apps}
  \resizebox{0.5\textwidth}{!}{%
  \begin{tabular}{|l|c|c|c|}
    \hline
    \textbf{Applications} & \textbf{Supervised} & \textbf{Unsupervised} & \textbf{Reinforcement} \\ \hline
    Traffic Prediction & $\cmark$ & $\cmark$ & $\xmark$ \\ \hline
    Congestion Control & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
    Anomaly Detection & $\cmark$ & $\cmark$ & $\xmark$ \\ \hline
    Channel Est. \& Equal. & $\cmark$ & $\xmark$ & $\xmark$ \\ \hline
    Network Optimization & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
    Routing & $\xmark$ & $\cmark$ & $\cmark$ \\ \hline
    Spectrum Management & $\xmark$ & $\xmark$ & $\cmark$ \\ \hline
    Handover Management & $\cmark$ & $\xmark$ & $\cmark$ \\ \hline
    Resource Allocation & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
    Physical Layer Security & $\cmark$ & $\cmark$ & $\xmark$ \\ \hline
  \end{tabular}
}
\end{table}
